Impact of network topology on the performance of Decentralized Federated Learning

Fully decentralized learning is gaining momentum for training AI models at the Internet's edge, addressing infrastructure challenges and privacy concerns. In a decentralized machine learning system, data is distributed across multiple nodes, with each node training a local model based on its respective dataset. The local models are then shared and combined to form a global model capable of making accurate predictions on new data. Our exploration focuses on how different types of network structures influence the spreading of knowledge - the process by which nodes incorporate insights gained from learning patterns in data available on other nodes across the network. Specifically, this study investigates the intricate interplay between network structure and learning performance using three network topologies and six data distribution methods. These methods consider different vertex properties, including degree centrality, betweenness centrality, and clustering coefficient, along with whether nodes exhibit high or low values of these metrics. Our findings underscore the significance of global centrality metrics (degree, betweenness) in correlating with learning performance, while local clustering proves less predictive. We highlight the challenges in transferring knowledge from peripheral to central nodes, attributed to a dilution effect during model aggregation. Additionally, we observe that central nodes exert a pull effect, facilitating the spread of knowledge. In examining degree distribution, hubs in Barabasi-Albert networks positively impact learning for central nodes but exacerbate dilution when knowledge originates from peripheral nodes. Finally, we demonstrate the formidable challenge of knowledge circulation outside of segregated communities.

==> old_netai.tex <==
% ER not idempotent
In ~\cref{fig:er_accuracy_tot} we show the evolution of the accuracy per node over time (each curve corresponds to one node). The top-row plots refer to the edge-focused case, where the digits in class G2 are assigned to leaf nodes, while the bottom-row plots correspond to the hub-focused scenario, where the well-connected nodes get all the images in G2. The first interesting result is that, in the edge-focused case, the separation between the curves of the nodes having more data and those that have fewer data is more evident. This means that when leaf nodes possess the missing classes (G2 images), it is harder for knowledge to circulate.
%
This finding holds when we vary $p$ (which increases from left to right). However, in the edge-focused scenario with below-critical $p$ (top left corner), we see that some nodes are eventually able to reach the accuracy of the nodes holding more data. But as we go from left to right, i.e., from less to more connected networks, this ability vanishes. This is quite interesting as well as counterintuitive. When the network is more connected, high-degree nodes (we refrain from calling them hubs, as in ER networks hubs do not exist) get proportionally more connected than leaf nodes. As G2 data are present only in leaf nodes, the additional connectivity plays against knowledge diffusion from leaves, as leaves' models are averaged among larger sets of nodes (due to higher degrees of more connected nodes), and therefore their knowledge ``weighs" less in the average. This is also clear in Figure~\ref{fig:er_accuracy_lessdata_hubshighlight}, where we show the accuracy only for nodes that are only assigned G1 images, and highlight the curves of the highest-degree nodes, which remain at low accuracy. The more the network is connected, the more high-degree nodes ``drag" other nodes toward their performance. In the hub-focused case (lower part of Figure~\ref{fig:er_accuracy_tot}) results are more intuitive, as the highest degree nodes enjoy higher accuracy, and are able to drag all the other nodes closer and closer to their performance.

In Figure~\ref{fig:er_mean_acc_std_all}, we aggregate the accuracy among all nodes in the same experiment and we show the evolution over time of the average and standard deviation of the accuracy. 
Coherently with Figure~\ref{fig:er_accuracy_tot}, the average accuracy in the edge-focus case is lower than in the hub-focus case. This is again due to high-degree nodes (in the former case) blocking the spreading of knowledge from leaves.
An interesting feature can be highlighted by comparing, in both cases, the standard deviation curves for networks below the critical threshold ($p = 0.03$, blue and orange curves in the figure) and the rest, which clearly show a lower rate of decay (after an initial increase). This can be attributed to the effect of longer paths when $p = 0.03$ (because the network is less connected), which hinders the alignment of local models across nodes, which are in this case farther away than for more connected networks (values of $p$ at and beyond the critical threshold). 
%
Also, the standard deviation values are generally higher in the edge-focus case, as hubs hinder other nodes to incorporate knowledge from leaves. This effect, again, is less pronounced for less connected networks, where some nodes are able to ``escape" the dragging effect of high-degree nodes, thus resulting in higher accuracy (but higher standard deviation) at the level of the entire network.

Finally, we can observe another overall effect by jointly analysing the accuracy per node, the average accuracy and the standard deviation for the edge-focus case. Specifically, \emph{on average} nodes in the least connected network achieve lower accuracy (Figure~\ref{fig:er_mean_acc_std_all}, orange and blue curves) even though, as a side effect of the higher standard deviation, some non-leaf nodes are able to increase their accuracy escaping the attraction effect of high-degree nodes. As the network becomes more and more connected, no node in the ``non-leaf and non-hub" class is able to reach the same accuracy, even though, on average, the overall accuracy increases. This means that, as a side effect of additional connectivity, hubs tend to increase their accuracy, even though they block other nodes to efficiently incorporate models of leaf nodes.

%For the mean accuracy plot, we see that the edges focus scenario is fairly below the hubs focus one. Both the scenarios show a visible separation between the accuracy belonging to the network having value of $p$ below the critical value and the ones above. Looking at the standard deviation plot, we can see that the edges focused scenarios show a higher standard deviation. Note that the edges focus scenario lines belonging to the networks of value $p$ above the critical value have standard deviation close, but with a slower decay rate, to the one of the hubs focus scenario with value $p = 0.03$. Thus, we argue that the slower decay rate comes from the average shortest path length. It, in fact, decrements drastically from values of $p$ below the critical value and the ones above. This means that the number of steps required to reach nodes far from each other is less in the second case. Therefore, the variability between nodes is more difficult to eliminate and requires more communication rounds.
\begin{figure*}[h!]
\hspace{-1cm}
    \includegraphics[width = 1.2\textwidth]{results_images/er_images/accuracy_tot.png}%\vspace{-10pt}
    \caption{Accuracy in ER networks (all nodes). From left to right: increasing values of $p$; from top to bottom: edge-focused scenario and hub-focused scenario.} %\vspace{-10pt}
    \label{fig:er_accuracy_tot}
\end{figure*}

\begin{figure}[h!]
\hspace{-1cm}
    \includegraphics[width = 1.2\textwidth]{results_images/er_images/accuracy_lessdata_edges_focus_hubs_highlight.png}%\vspace{-10pt}
    \caption{Accuracy in ER networks (nodes with only G1 images, edge-focused scenario), curves of the high-degree nodes in red.}
    \label{fig:er_accuracy_lessdata_hubshighlight}
    % \vspace{-10pt}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width = \textwidth]{results_images/er_images/mean_acc_std_all.png}%\vspace{-10pt}
    \caption{ER (all nodes): accuracy mean and std.}
    \label{fig:er_mean_acc_std_all}
    % \vspace{-10pt}
\end{figure}

==> parts_of_main/focus_section.tex <==
\section{DecAVG update and degree relationship}
This section is devoted to displaying some of the analysis' observations concerning the interactions between degree and other centrality metrics.  Generally speaking, we have observed that the G1 nodes' performances fall into distinct groups depending on the amount of connections they have with the highly informative G2 nodes. Intuitively, a positive correlation emerges, indicating that higher connectivity to these informative nodes aligns with improved performance. 
This is insufficient on its own, though, because the DecAVG method also has a dilution impact dependent on the nodes' degrees, meaning that the more degrees a node has, the more models it will average. The DecAVG update mechanism, by design, entails averaging among all incoming models. Consequently, with a constant number of connections to the most informative nodes. The higher degree translates to a greater number of non-informative updates.
To shed light on this interaction, we emphasise two particular cases. The Erdos-Renyi (ER) network is examined first, using the betweenness centrality measure in the lowest focus scenario.  In addition, we investigate the Barabási-Albert (BA) network in the lowest focus setting by using the clustering coefficient metric. This focused analysis reveals the complex dynamics at work, providing insight into how node degree and the DecAVG scheme interact to determine the overall performance in these particular network configurations.

\subsection{ER}
In \Cref{fig:er_bet_highlight} we show the accuracy levels for all G1 nodes of the ER idem(2) for the betweenness centrality in the lowest focus case. On the left, the curves are colored according to their connections to the most informative nodes. With the lowest value color belonging to the class of nodes with no direct connection to the G2 nodes. We can observe a clear separation in the performances, based on the amount of connections to the G2 nodes. 
On the right, we highlighted in red the nodes with degree values higher than the 90th percentile of the G1 nodes. As we can see, and as expected from the proportionality with the degree measure, the high-degree nodes are all placed in the lowest part of the curves, however, the few of them that have a higher number of connections to the G2 nodes exhibit higher accuracy levels. Thus showing the interplay between the averaging update and degree.
\begin{figure}[ht!]
    \centering
    \includegraphics[width=\textwidth,height =1.2\textheight,keepaspectratio]{results_images/er_images/bet_highlight.png}
    \caption{Accuracy levels of all G1 nodes for the ER idem(2) in the lowest focus case of the betweenness centrality data distribution. Left: accuracy levels of G1 nodes colored by the number of links to G2 nodes; right: same curves with high-degree nodes highlighted in red.}
    \label{fig:er_bet_highlight}
\end{figure}%

\subsection{BA}
Similarly, in \Cref{fig:ba_clust_highlight} we show the accuracy levels of all G1 nodes of the BA with $m=2$ for the clustering coefficient in the lowest focus case. As above, on the left, we present the curves of G1 nodes colored according to the number of connections they have to the G2 nodes. Also here there is a group separation, although less well-defined for nodes with more than 1 direct connection. On the right, again, we highlighted the nodes taken from the 90th percentile of G1 nodes with high degree values. As we can see, the nodes with no direct connection to the most informative nodes are among the ones with the lowest accuracy levels, however if one were to have a direct connection it would result in a considerably higher accuracy level. 
\begin{figure}[ht!]
    \centering
    \includegraphics[width=\textwidth,height =1.2\textheight,keepaspectratio]{results_images/ba_images/clust_highlight.png}
    \caption{Accuracy levels of all G1 nodes for the BA with $m=2$ in the lowest focus case of the clustering coefficient data distribution. Left: accuracy levels of G1 nodes colored by the number of links to G2 nodes; right: same curves with high-degree nodes highlighted in red.}
    \label{fig:ba_clust_highlight}
\end{figure}%
